Uncertainty Averse Pushing with Model Predictive Path Integral Control

Planning robust robot manipulation requires good forward models that enable robust plans to be found. This work shows how to achieve this using a forward model learned from robot data to plan push manipulations. We explore learning methods (Gaussian Process Regression, and an Ensemble of Mixture Density Networks) that give estimates of the uncertainty in their predictions. These learned models are utilised by a model predictive path integral (MPPI) controller to plan how to push the box to a goal location. The planner avoids regions of high predictive uncertainty in the forward model. This includes both inherent uncertainty in dynamics, and meta uncertainty due to limited data. Thus, pushing tasks are completed in a robust fashion with respect to estimated uncertainty in the forward model and without the need of differentiable cost functions. We demonstrate the method on a real robot, and show that learning can outperform physics simulation. Using simulation, we also show the ability to plan uncertainty averse paths.

==> results.tex <==
%We now present some preliminary results. Figure~\ref{fig:ensembleResults} (left column) shows five data sets generated in a Box2D environment of size 10m x 10m. The start and end locations of the pushes are shown in Figure~\ref{fig:data_box2d_experiments}. To generate this a set of random locations with some excluded areas were chosen and random impulse forces were applied to the object at random push locations on the surface. The data is collected as [current state, action, next state]. This data is used to train an ensemble of MDNs. The trained MDNs are tested with test points generated within the same state-action space. The average uncertainty at a location is calculated by sampled averages performed in a  10m x 10m grid---see Figure~\ref{fig:ensembleResults} (right column). One can see that the ensemble approximately matches the collected data space. Blue represents areas of low uncertainty and red areas denote areas of high uncertainty. The parameters of the network used to learn from these different data sets are the same. 

%\begin{figure}[!th]
%\centering
%\includegraphics[width=0.4\textwidth]{data_box2d_experiments.png}
%    \caption{This shows green and red crosses as the starting and final locations, respectively, for the pushes. A total of 380 pushes were collected using the Box2D simulator, with 20 pushes per start location. Pushes had a random direction and fixed magnitude.}
%    \label{fig:data_box2d_experiments}
%\end{figure}


%\begin{figure}[!th]
%\centering
%\includegraphics[width=0.4\textwidth]{unc_calibration_figs/robot_data/robot_data_and_unc_calibration.png}
%    \caption{Data and corresponding uncertainty heat-map from robot push data.}
%    \label{fig:real_data_experiment}
%\end{figure}
Next, we show the performance, given an MDN model trained on this data, of a path integral based model predictive controller (Algorithm 1) to find a set of commands to push the object to the goal. In this case the look-ahead for MPC is merely two steps. %Initially the policy is applied with point mass assumption, i.e the push locations are always the centre of mass of the object and one needs to find the set of force components along X and Y axis that would push the object towards the target. 
Figure~\ref{fig:unc_tradeoff_experiment_off} shows, when there is no uncertainty penalty, that it moves the box towards the goal in an almost straight line. Figure~\ref{fig:unc_tradeoff_experiment_on} shows the same set up, but now with a penalty and so the planner tries to avoid the region while moving towards the goal. 


\begin{figure}[!th]
\centering
\includegraphics[width=0.4\textwidth]{unc_off_exp/experiment_2/figure_1.png}
    \caption{Performance of Algorithm 1. Without an uncertainty penalty, the box tends to follow a straight line (dark blue) towards target, ignoring uncertainty. Multi-coloured lines are forward sampled trajectories form the current box state, and circle radius represents current region uncertainty.  }
    \label{fig:unc_tradeoff_experiment_off}
\end{figure}


\begin{figure}[!th]
\centering
\includegraphics[width=0.4\textwidth]{unc_on_exp/experiment_2/figure_1.png}
    \caption{Performance of Algorithm 1. Penalizing uncertainty, the box is deflected towards regions with lower uncertainty, as shown by the trajectory depicted in dark blue. The heuristic cost is defined such that uncertainty acts as a penalty for 150 pushes, and is set to zero afterwards ($\gamma = 0$). For this experiment gamma was $\gamma = 115$, $R = \mathbf{I} 0.17$, $h = 2.0$, $\rho = 2.0$, $N = 2$, $\Delta t = 0.05$, $K = 10$. As before, the multi-coloured lines are forward sampled trajectories form the current box state, and circle radius represents current region uncertainty.}
    \label{fig:unc_tradeoff_experiment_on}
\end{figure}


\begin{figure}[!h]
\label{fig:traj_follow_algorithm2}
\includegraphics[width=0.48\textwidth]{unc_on_exp/experiment_1/image_traj_follow.png}
\caption{Performance of Algorithm 2. In this case the red dots represent the waypoints on the trajectory found by Algorithm 2. This minimises uncertainty while staying within a fixed distance of the optimal trajectory if there were no uncertainty. Algorithm 1 is then used to reach each waypoint in turn (white line). Forward sampled trajectories form the current box state are shown as multi-coloured lines, and circle radius represents current region uncertainty.}
\end{figure} 

 %Without uncertainty penalty, point mass particle tends to follow a straight line towards target, ignoring uncertainty. Penalizing uncertainty heuristically. Uncertainty is used as penalty for fixed number of steps and switched off afterwards. The point mass particle is deflected towards regions with lower uncertainty, after the maximum number of steps is reached, undcertainty penalisation is switched off, from which point the point max goes directly to the goal.

